Adaptive Coverage Path Planning for Efficient Exploration of Unknown Environments

We present a method for solving the coverage problem with the objective of autonomously exploring an unknown environment under mission time constraints. Here, the robot is tasked with planning a path over a horizon such that the accumulated area swept out by its sensor footprint is maximized. Because this problem exhibits a diminishing returns property known as submodularity, we choose to formulate it as a tree-based sequential decision making process. This formulation allows us to evaluate the effects of the robot's actions on future world coverage states, while simultaneously accounting for traversability risk and the dynamic constraints of the robot. To quickly find near-optimal solutions, we propose an effective approximation to the coverage sensor model which adapts to the local environment. Our method was extensively tested across various complex environments and served as the local exploration algorithm for a competing entry in the DARPA Subterranean Challenge.

==> 3_Preliminaries.tex <==

The Partially Observable Markov Decision Process (POMDP) is a general framework for sequential decision-making when the current state is not perfectly observable by the robot.  A POMDP is described as a tuple $\langle \mathbb{S}, \mathbb{A}, \mathbb{Z}, T, O, R \rangle$, where $\mathbb{S}$ is the set of joint robot-and-world states, $\mathbb{A}$ and $\mathbb{Z}$ are the set of robot actions and observations.  At every time step, the agent performs an action $a \in \mathbb{A}$ and receives an observation $z \in \mathbb{Z}$ resulting from the robot's perceptual interaction with the environment.
The motion model $T(s, a, s') = p(s'\,|\,s, a)$ defines the probability of being at state $s'$ after taking action $a$ at state $s$. The observation model $O(s, a, z) = p(z\,|\,s, a)$ is the probability of receiving observation $z$ after taking action $a$ at state $s$. The reward function $R(s, a)$ returns the expected utility for executing action $a$ at state $s$.

In a POMDP, it is assumed that the state is not perfectly observable. Rather, the robot only has access to an observation $z \in \mathbb{Z}$ that provides partial information about the current state. 
With only partial state knowledge, the robot must consider a complete history of past actions and observations:
\begin{align}
    h_t = \{ a_0, z_1,...,z_{t-1}, a_{t-1}, z_t \ .\}
\end{align}
The belief state, $b_t$, is an effective way of capturing $h_t$. At time $t$, the belief $b_t$ is a posterior distribution over states conditioned on the initial belief $b_0$ and the past action-observation sequence:
\begin{align}
    b_{t} = p(s \,|\, b_0, a_{0:t-1}, z_{1:t})\ .
\end{align}

A POMDP can be formulated as a \emph{belief MDP}, or a Markov decision process where every state is a belief. A belief MDP is described as a tuple $\langle \mathbb{B}, \mathbb{A}, \tau, r \rangle$, where $\mathbb{B}$ is the set of belief states over the POMDP states, $\mathbb{A}$ is the set of robot actions, $\tau(b, a, b') = p(b'\,|\,b, a)$ is the belief state transition function, and the reward function $r(b,a)$ returns the utility for executing action $a$ in belief $b$. 

\note{If you keep the POMPDP story, then you'll want to add some POMDP references to the next paragraph.}

A solution to a POMDP is a policy that maps beliefs to actions. The optimal policy is one that maximizes the expected cumulative reward. Due the computational complexity of POMDPs, they cannot be solved exactly in real-time. Online POMDP algorithms approximate the optimal policy by reasoning over the states reachable from the current belief state over a finite horizon. Common online methods use a Monte Carlo tree search (MCTS) approach that simulates, or \emph{rolls out}, action-observation sequences according to a provided rollout policy. Given a generative model (or a black box simulator) for discrete action and observation spaces, MCTS learns the value function of the reachable belief subspace with an adequate exploration-exploitation trade-off.




==> 4_Problem_Formulation_POMDP.tex <==
\begin{figure}[t]
  \centering
  \subfloat[Continuous Observation]{\label{fig:a}\includegraphics[width=.22\textwidth]{figures/continuous_fov.png}}
  \; \;
  \subfloat[Discretized Observation]{\label{fig:b}\includegraphics[width=.22\textwidth]{figures/discretized_fov.png}} 
  
  \subfloat[Non-Diagonal Action $a_{1}$]{\label{fig:a}\includegraphics[width=.235\textwidth]{figures/non_diag_action_crop2.png}}
  \,
  \subfloat[Diagonal Action $a_{\sqrt{2}}$]{\label{fig:b}\includegraphics[width=.235\textwidth]{figures/diag_action_crop2.png}}     
  \caption[The short caption]{
  Simulated observation, Eq.~(\ref{eq:cov_prob}), returned by an omnidirectional range finder coverage sensor, displayed as a continuous measurement (a), and a discretized measurement over the lattice graph world representation (b). The diffused color map mimics the coverage probability curve-- darker shades indicate higher coverage probabilities. The marginal coverage after a non-diagonal action (c) and diagonal action (d) is represented by the shaded gray cells. Note that the ratio of marginal coverage to distance traveled over the lattice is not equivalent for non-diagonal and diagonal actions: $I(s^o, a_{\sqrt{2}})/d_{ij} \neq I(s^o, a_{1})/d_{ij}$, where $s^o$ indicates a risk-free world. We address this discrepancy with Eq.~(\ref{eq:distance_weight}).
  }
  \label{fig:adapt_cartoon}
\end{figure}

\note{Somewhere in this section or the next, you should discuss how the regions beyond the frontiers are properly 
\note{Note that the problem of efficiently covering nodes in a graph is unfortunately also called the "Shortest Covering Path" \cite{SCCP}.  } 

We assume that the environment can be divided into sufficiently small cells such that when the robot is positioned in the cell, it can cover all terrain modeled by that cell.  Hence, we can model a known environment by an abstract graph structure $G = (N, E)$, with free and occupied nodes $N_{free}\cup N_{occ} = N$, the traditional coverage problem aims to find a sequence of nodes and edge traversals that pass through all free nodes $N_{free} \subseteq N$.  By incorporating a coverage sensor footprint $F:N\rightarrow \mathcal{V}(N)$, which maps each node to a subset of ``covered'' nodes, and adding the objective of minimizing travel distance, the coverage problem can be seen as generalization of the traveling salesman problem -- \emph{orienteering problem}. 
The objective of the traditional orienteering problem is to determine the path $p$ through a subset of nodes $p = \{n_0, .., n_N\} \subseteq N_{free}$ such that the number of free nodes within the accumulated sensor field-of-view is maximized, subject to a budget constraint: 
\begin{equation}
\label{eq:modular}
\begin{aligned}
    &p^* = \argmax_{p} \; \sum_{n_i \in p} \, F(n_i), \\
    &\text{subject to} \quad \ell(p) \leq B, 
\end{aligned}
\end{equation}

\noindent where $\ell(p)$ is the length of the path and $B$ is a user-defined travel budget. The modular orienteering formulation Eq.~(\ref{eq:modular}) assumes additive reward, which isn't compatible with the coverage problem where the marginal benefit of appending the path with a node $n_2$ ``close'' to $n_1 \in p$ is less than that if $n_2 \not\in p$. This \emph{diminishing returns} property is termed submodularity \cite{?}. To formulate the submodular orienteering problem, we define the reward as the marginal coverage given all the previously traversed nodes:
\begin{align}
    \label{eq:marg}
     \tilde{F}(n_i) = F(n_i \, | \, {n_0, .., n_{i-1}}).
\end{align}
\noindent Then the submodular orienteering problem is as follows:
\begin{equation}
\label{eq:submodular}
\begin{aligned}
    &p^* = \argmax_{p} \; \sum_{n_i \in p} \, \tilde{F}(n_i), \\
    &\text{subject to} \quad \ell(p) \leq B.
\end{aligned}
\end{equation}

\noindent Next, we model the submodular orienteering problem as a discrete-time decision making process where the optimal path is a sequence of actions that maximizes an expected cumulative coverage reward.
Then, we employ an MCTS-based online solver that finds near-optimal coverage paths by efficiently simulating how the robot interacts with the world using an adaptive coverage model. 
We incorporate a hard path length budget by limiting the depth of the tree search.


  


==> 5_Methodology_POMDP.tex <==
\blue{[Change to MDP]}
We frame the submodular orienteering problem as a Partially Observable Markov Decision Process (POMDP) where the problem objective is directly expressed in terms of the coverage uncertainty on the environment state. 
That is, the belief encodes the robot's knowledge about the environment, 
and the marginal coverage reward associated with adding a node to an existing path is an explicit function of this belief. 
Hence, we model our POMDP as a belief MDP, i.e. a Markov decision process with a belief-dependent reward function $r(b,a)$.
\subsection{World Representation}
We approximate the local world state by an information-rich graph structure called the Information Roadmap (IRM) \cite{sungpilgrim}. The IRM is a fixed-size lattice $G = (N, E)$ with nodes $N$ and edges $E$. 
It is a rolling map centered at the robot's current position. 
Nodes represent discrete areas in space, and edges represent actions. 
To construct $G$, we uniformly sample nodes $n_i \in N$ in a neighborhood of the robot, and compute the traversability risk and coverage probability distribution over a discrete patch centered at each node, i.e., $p_r(n_{i})$ and $p_c(n_{i})$, which are stored as node properties. 
For scalability, we bin node traversability risk probabilities into three groups: occupied $p_r(n_{i})=1$, unknown $p_r(n_{i})=0.5$, and free $p_r(n_{i})=0$.    
For an edge $e_{ij} \in E$, we compute and store the traversal distance $d_{ij}$ and traversal risk $\rho_{ij}$ between two connected nodes. 
In summary, the IRM provides an estimate of: \textit{(i)} the traversability risk of the world with respect to a robot's dynamic constraints (risk traversal map $\{ p_r(n_{i}) \}$), and \textit{(ii)} what parts of the world have been observed, or \textit{covered}, by a particular sensor (coverage map $\{ p_c(n_{i}) \}$).

\begin{figure}[t]
  \centering
  \subfloat[Pessimistic Coverage Model (Deterministic) ]{\label{fig:a}\includegraphics[width=.45\textwidth]{figures/small_fov_combined.png}}
  \; \;
  \subfloat[Optimistic Coverage Model (Deterministic)]{\label{fig:b}\includegraphics[width=.45\textwidth]{figures/big_fov_combined.png}} 
  
  \subfloat[Proposed Probabilistic Coverage Model]{\label{fig:a}\includegraphics[width=.45\textwidth]{figures/prob_fov_combined.png}}

  \caption[The short caption]{\blue{[REMOVE?]} Illustrative example of the effect of different simulated coverage observations on exploration efficiency and completeness: pessimistic observation where the coverage range underestimates true range (a), optimistic observation where the coverage range overestimates true range (b), and our proposed probabilistic observation (c). With the pessimistic model, the robot uncovers the narrow channel after executing an inefficient ping-pong trajectory, which poses undue risk given its occasional proximity to obstacles. Alternatively, the optimistic model leads to an efficient path down the centerline of the cavern, but the robot fails to detect the narrow channel and terminates exploration early. Our proposed probabilistic model combines the benefits of pessimistic and optimistic coverage. The robot travels down the centerline, sparsely covering the main cavern until it encounters the end. At this point, it densely covers the space and exposes the narrow channel.}
  \label{fig:prob_cartoon}
\end{figure}

\subsection{Formulation}

\ph{State}
The robot-world state is defined as $s = (q, W)$, where $q$ is the robot state and $W$ is the world state. We define $q$ and $W$ in terms of the IRM. The robot state $q=(n_q, \mu)$, where $n_q$ is the node closest to the robot's current location, and $\mu$ is the robot's heading direction, defined with respect to the lattice geometry. The world state  $W = G$, where $G$ is the IRM containing traversability risk and coverage world state estimates.

\ph{Action}
We define an action $a$ as the robot motion control from a node $n_i \in N$ to a neighboring node $n_j \in N$, along an edge $e_{ij} \in E$. 
A node is directly connected to its eight neighbors, discretizing the valid action space for a single state into movement along the four cardinal/non-diagonal (N, E, S, W) and four intercardinal/diagonal (NE, SE, SW, NW) directions. We denote actions along the cardinal and intercardinal directions by $a_{\sqrt{2}}$ and $a_{1}$, respectively. 
We define the robot's heading direction $\mu \in (N, E, S, W, NE, SE, SW, NW)$.


\ph{Robot Dynamics}
We approximate the robot motion model $T(q, a, q')$ as deterministic. 
Given an action $a$ directing traversal of edge $e_{ij}$, the robot will reach node $n_j$ with probability 1.
Actions that cause the robot to leave the bounds of $G$ 
or enter nodes that are unknown or occupied, $p_r(n_{i}) = 0.5$ or $1$,
have no effect.

\ph{Coverage Sensor Model}
A coverage observation $z$ is defined to be the the measurement returned from our coverage sensor -- an omnidirectional range finder. We use the terms \emph{observe} and \emph{cover} interchangeably when discussing the sensor measurement. 
The robot covers nodes within its line-of-sight, computed using ray-tracing techniques on the traversal risk map $\{ p_r(n_{i}) \}$ in combination with sensor range constraints. See $\text{\senseFunc}$ in Alg.~\ref{alg:sense}. To account for increasing ray sparsity in the radial direction, we compute the coverage probability for a node as a function of the robot-to-node distance. Given the robot node $n_q$, a node $n_i$ is covered with probability $P_{\text{cov}}(n_i | \; n_q)$. We heuristically model the coverage probability $P_{\text{cov}}$ as an S-shaped logistic function: 
\begin{align}
\label{eq:cov_prob}
    P_{\text{cov}}(n_i | \; n_q) = \frac{1}{1+e^{k \, (r_i-r_0)}},
\end{align}
\noindent where $r_{i}$ is the euclidean distance between the robot node $n_q$ and node $n_i$, and constants $r_0$ and $k$ are the sigmoid's midpoint and steepness, respectively. 

The coverage probability distribution over the radial distance from the center of the sensor in shown in
Fig.~\ref{fig:overlap}. The probabilistic sensor model plays a crucial role in efficiently exploring an environment when the fundamental objective is constructing a map of the environment. Fig.~\ref{fig:prob_cartoon} illustrates how a probabilistic coverage model, opposed to deterministic ones, helps quickly expose large topological features in the environment by modulating coverage density based on the local geometry. \blue{[very hand wavy - need to formalize it?]}

\ph{World Dynamics}
We assume independence between sensor measurements. Therefore, to integrate new measurements (line 5 in Alg.~\ref{alg:sense}), we compute the maximum of the old and new coverage probability, which yields a optimistic estimate of coverage for that node. 

\input{alg_obs}


\ph{Reward Function}
We now redefine our marginal coverage from Eq.~(\ref{eq:marg}) to be the uncertainty reduction in the world coverage state induced by an action:
\begin{align}
\label{eq:margCov}
    &I(s, a) = \sum_{n_i \in N} \beta \Big( p_c(n_{i} \, | \, a) - p_c(n_{i}) \Big),
    \\[10pt]
    &\text{where} \; \; \beta = 
    \begin{cases}
    w_{\text{1}}, \; \; \; \text{if} \; \; p_r(n_{i}) = 0.5
    \\[2pt]
    w_{\text{2}}, \; \; \; \text{otherwise},
    \end{cases}
\end{align}
\noindent where constants $w_{1}$ and $w_{2}$ weight the value received by covering known and unknown nodes, respectively. As $w_{1} < w_{2}$, the constant $\beta$ encourages the robot to plan actions that cover nodes with a known occupancy. 


  



The reward function is defined as a weighted sum of marginal coverage and action penalties:
\begin{align}
\label{eq:reward}
    &R(s, a) = k_I \, I(s, a) - \big[ k_d \, d_{ij} + k_{\rho} \, \rho_{ij} + k_{\mu} \, \Delta_{\mu} \big], 
\end{align}
\noindent where $d_{ij}$ is the traversal distance, $\rho_{ij}$ traversal risk, and $\Delta_{\mu}$ is the cost of rotation due to the robot's non-holonomic constraints. Constants $k_I$, $k_d$, $k_\rho$, and $k_\mu$ weigh the importance of coverage, traversal distance, risk, and motion primitive history on the total reward.

Given a coverage sensor with a circular field-of-view, the uncovered area after a diagonal and non-diagonal action should scale equivalently with distance traveled. However, since Eq.~(\ref{eq:marg}) is evaluated over a discretized space $G$, the ratio of marginal coverage to distance traveled is not equivalent for all actions on the lattice, as illustrated in Fig.~\ref{fig:overlap}. Given this marginal coverage discrepancy between actions, we define $k_d$ as a function of coverage parameters in order to ensure non-diagonal and diagonal actions are equally rewarding; that is, $R(s,a_1) = R(s,a_{\sqrt{2}})$ for the same $\rho_{ij}$ and $\Delta_{\mu}$. If $h$ is the height dimension of a grid cell in $G$, then we define $k_d$ as: 
\begin{align}
\label{eq:distance_weight}
    k_d = \frac{k_I}{h} \cdot \frac{I(s^o, a_{\sqrt{2}}) - I(s^o, a_{1})}{(1-\sqrt{2})}
\end{align}
\noindent where state $s^o$ denotes a risk-free world where the only covered region is aligned with the robot's current sensor footprint. 


\ph{Optimal Policy}
It is fundamentally infeasible to solve an unknown environment coverage problem over an infinite horizon since information about the world is incomplete, and often inaccurate, at runtime. Instead, in such domains, a Receding Horizon Planning (RHP) scheme has been widely adopted as the state-of-the-art \cite{bircher2016receding}. The optimal policy with RHP is:
\begin{align}
  \pi_{t:t+T}^*(s) &= \argmax_{\pi \in \Pi_{t:t+T}} \, \sum_{t'=t}^{t+T} \gamma^{t'-t} R(s_{t'}, a_{t'}),
  \label{eq:receding_objective_function}
\end{align}
where $T$ is a finite planning horizon for a planning episode at time $t$.
Given the policy from the last planning episode, only a part of the optimal policy, $\pi^*_{t:t+\Delta t}$ for $\Delta t \in (0, T]$, will be executed at runtime. A new planning episode will start at time $t+\Delta t$ with updated robot-world state.

\subsection{Online Planning}
In order to solve Eq.~(\ref{eq:receding_objective_function}), we use Monte Carlo tree search (MCTS) \cite{browne2012survey}.
During every planning episode, a lookahead tree is iteratively constructed by simulating action-observation sequences using a random rollout policy $\pi_{rollout}$. 
During a single iteration, rollouts and tree expansion stop when a predefined depth, or our path budget, is reached.
Given a state $s$ and action $a$, a generative model $\mathcal{G}$ (i.e. the black box simulator of the MDP) provides a sample successor state $s'$, observation $z$, and reward $r$. 
Since we do not have access to the ground truth state of the environment, our generative model is an estimate based on the most recent robot sensor measurements used to construct the world representation $G$.
POMCP terminates after reaching a user-defined maximum number of simulations.
Then, the action with the highest estimated value $\max_{a}Q(s,a)$ is sent to the robot for execution.

\input{alg_planner}


\ph{Adaptive Coverage Observation} 
While MCTS is an anytime algorithm, meaning construction of the tree can terminate at any point and a solution will be recovered, it only converges to the optimal solution with a sufficient number of simulations.
Although it may be infeasible to reach the optimal solution given time constraints, estimates of the action values become increasingly more reliable with more simulations, leading to a higher quality coverage path. 
In order to find quality solutions at high planning rates, a real-time system 
must find a good balance between the fidelity of a simulation (e.g. how accurately we model the coverage observation) and the number of simulations. 

To maximize the number of simulations within a suitable planning time, we propose an approximation of the observation $z$, computed in Alg.~\ref{alg:sense}, that reduces the time complexity of the generative model $\mathcal{G}$. Our approximate observation obviates the need for expensive ray-tracing operations. 
First, we estimate the spaciousness $r_{\text{spac}}$ of the local environment, and then we adapt the distance at which a range-finder coverage measurement is performed based on $r_{\text{spac}}$. 
We denote this adaptive coverage range by $r_{\text{adapt}}$.

\blue{[WIP]}
Given a range-finder 3D pointcloud scan $\{ z_i \}$, we compute spaciousness as:

\begin{equation}
    r_{\text{spac}} = f(\text{median}[\{z_i\}]) \,, \\
\end{equation}
\noindent where $\text{median} [\{ z_i \}]$ is the median euclidean point distance from the range-finder origin to each point in $\{ z_i \}$, and $f$ is a low-pass filter: $f(x_t)=\alpha_1 \, f(x_{t-1}) + \alpha_2 \, x_{t}$ with constants $\alpha_1=0.95$ and $\alpha_2=0.05$.

We similarly define a local environment's \textit{density} as 
\begin{equation}
    r_{\text{den}} = g(D[\{z_i\}]) \,, \\
\end{equation}
\noindent where $g$ is a low-pass filter: $g(x_{t}) = \beta_1 \, g(x_{t-1}) + \beta_2 \, x_t$ and $D[\{z_i\}]$ computes the average per-point distance to $N$ nearest neighbors of that point, such that
\begin{equation}
    D[\{z_i\}] = \frac{1}{|\{z_i\}|} \sum_{z_j \in \{z_i\}} \left\{ \frac{1}{|\{z_n\}|} \sum_{z_k \in \{z_n\}_N} \left\| z_j - z_k \right\| _2 ^2   \right\}
\end{equation}

$Z = \{ z_1, z_2, ..., z_N \}$

where $N(z_i) = \{ : d() \}$

Both $r_\text{spac}$ and $r_\text{den}$ provide our system with a notion of the local environment's size but through different means. Intuitively, $r_\text{spac}$ is the robust middle observation of the radius of point distances, which is smaller in value for small-scale environments and larger for more expansive locations. On the other hand, $r_{\text{den}}$ tells us how close or far apart the points in a cloud are. Due to how modern 3D range-finders operate, for smaller environments, such points will be packed closer to each other, whereas the converse is true for large-scale locations. We combine these two methods such that
\begin{equation}
    r_{\text{adapt}} = \frac{r_{\text{spac}}}{r_{\text{den}}}^2 \,, \\
\end{equation}
\noindent where $r_{\text{adapt}}$ is lower-bounded at $1m$ and upper-bounded at $10m$. 

Equipped with $r_{\text{adapt}}$, we generate a probabilistic coverage mask $\{m_{i,c} \}$ (see \#1 in Alg.~\ref{alg:planner}). The mask serves as an input to the generative model, econGEN in Alg.~\ref{alg:GenModels}, which then computes the coverage observation $z$ using inexpensive matrix operations. In comparison, expGen in Alg.~\ref{alg:GenModels} uses the more exact, but significantly more expensive, Observation function in Alg.~\ref{alg:sense} when generating an coverage observation on line 3.






\blue{[Talk about cartoon of different models.]}




\input{alg_gen}



==> alg_gen.tex <==

\begin{algorithm}[h!]
\small
\caption{Estimated Generative Models $\mathcal{G}$}
\label{alg:GenModels}

\hspace*{1em}\underbar{\textbf{Function econGEN}}  $\triangleright$ economical model \\
\hspace*{1em}\textbf{Input: }state \state \\
\hspace*{1em}\hspace*{3.1em}coverage mask $\{ m_{i} \}$ \\
\hspace*{1em}\hspace*{2.8em} policy $\pi$ 
\begin{algorithmic}[1]
\STATE $n'_q, \, \mu' \gets \pi(n_q, \mu)$ %
\STATE $\{ p_c(n_{i})' \}  \gets \{ \text{max}\big[m_{i}, \; p_c(n_{i}) \big] \}$ $\triangleright$ fast
\STATE $r \gets R(s, a)$ $\triangleright$ Eq.~(\ref{eq:reward})
\RETURN $s', r$ %
\end{algorithmic}

\vspace*{0.1em}

\hspace*{1em}\underbar{\textbf{Function expGEN}} $\triangleright$ expensive model \\
\hspace*{1em}\textbf{Input: }state \state \\
\hspace*{1em}\hspace*{3.1em}coverage mask $\{ m_{i} \}$ \\
\hspace*{1em}\hspace*{2.8em} policy $\pi$ 
\begin{algorithmic}[1]
\STATE $n'_q, \, \mu' \gets \pi(n_q, \mu)$ %
\STATE $\{ p_c(n_{i})' \} \gets \text{\senseFunc}(n_q, G, r_{\text{max}})$ $\triangleright$ Alg.~\ref{alg:sense}, slow
\STATE $r \gets R(s, a)$ $\triangleright$ Eq.~(\ref{eq:reward})
\RETURN $s', r$ %
\end{algorithmic}

\end{algorithm}

==> alg_gen_POMDP.tex <==

\begin{algorithm}[t!]
\small
\caption{Estimated Generative Models $\mathcal{G}$}
\label{alg:GenModels}

\hspace*{1em}\underbar{\textbf{Function econGEN}}  $\triangleright$ economical model \\
\hspace*{1em}\textbf{Input: }state \state \\
\hspace*{1em}\hspace*{3.1em}coverage mask $\{ m_{i,c} \}$ \\
\hspace*{1em}\hspace*{2.8em} action $a$ 
\begin{algorithmic}[1]
\STATE $n'_q, \, \mu' \gets \pi(n_q, \mu)$ %
\STATE $\{ p(n'_{i,r}) \} \gets \{ p(n_{i,r}) \}$ %
\STATE \blue{[OPT A]} $z=\{ p(n'_{i,c}) \}  \gets \{ \text{max}\big[m_{i,c}, \; p(n_{i,c}) \big] \}$ $\triangleright$ fast
\STATE \blue{[OPT B]} $z  \gets \{ \text{max}\big[m_{i,c}, \; p(n_{i,c}) \big] \}$ $\triangleright$ fast %
\STATE $r \gets R(s, \pi)$ $\triangleright$ Eq.~(\ref{eq:reward})
\RETURN $s', z, r$ %
\end{algorithmic}

\vspace*{0.1em}

\hspace*{1em}\underbar{\textbf{Function expGEN}} $\triangleright$ expensive model \\
\hspace*{1em}\textbf{Input: }state \state \\
\hspace*{1em}\hspace*{2.8em} maximum sensor range $r_{\text{max}}$ \\
\hspace*{1em}\hspace*{2.8em} action $a$ 
\begin{algorithmic}[1]
\STATE $n'_q, \, \mu' \gets \pi(n_q, \mu)$ %
\STATE $\{ p(n'_{i,r}) \} \gets \{ p(n_{i,r}) \}$ %
\STATE \blue{[OPT A]} $z=\{ p(n'_{i,c}) \} \gets \text{\senseFunc}(n_q, G, r_{\text{max}})$ $\triangleright$ slow %
\STATE \blue{[OPT B]} $z \gets \text{\senseFunc}(n_q, G, r_{\text{max}})$ $\triangleright$ slow %
\STATE $r \gets R(s, \pi)$ $\triangleright$ Eq.~(\ref{eq:reward})
\RETURN $s', z, r$ %
\end{algorithmic}

\end{algorithm}








==> alg_planner.tex <==


\begin{algorithm}[t!]
\small
\caption{Coverage Planner}
\label{alg:planner}
\begin{algorithmic}
\STATE \underbar{\textbf{Function CoveragePlan}}
\REPEAT
    \item \textbf{Obtain: }state \state \\ %
    \hspace*{3.3em} pointcloud scan $\{ z_i \}$ \\
    \STATE \textbf{\#1 Generate Coverage Mask}
    \STATE Compute adaptive coverage range $r_{\text{adapt}}$ in Eq.~(\ref{eq:adapt})
    \STATE $\{m_{i} \} \gets \text{\senseFunc}(n_q, O,  r_{\text{adapt}})$
    \item \hspace*{2em} $\triangleright$ where $O \Rightarrow p_c(n'_{i}) = p_r(n'_{i}) = 0 \; \forall \; n_i \in N$
    \STATE \textbf{\#2 Find Planning Root}
    \STATE $n_{\tau}, \mu_{\tau} \gets \text{PathRoot}(s, a^{-}_{1:N})$ $\triangleright$ see PLGRIM in \cite{sungpilgrim}
    \STATE $s \gets (n_{\tau}, \mu_{\tau}, G)$ $\triangleright$ update robot state to root parameters
    \STATE \textbf{\#3 Plan and Execute}
    \item $T_r \gets \textsc{MCTS}(s, \; \{m_{i} \})$
    \item Extract action sequence $a^*_{1:N}$ from $T_r$ %
    \STATE \textbf{\#4 Prep for Next Episode}
    \item $a^{-}_{1:N} \gets a_{1:N}$ 
\UNTIL timeout
\end{algorithmic}


\vspace*{0.1em}


\begin{algorithmic}
\STATE \underbar{\textbf{Function PathRoot}}
\STATE \textbf{Input: }state \state \\
\hspace*{2.8em} previous action sequence $a^{-}_{1:N}$ \\
\vspace*{0.25em}
\STATE Extract path $a^{-}_{Q:N}$ $\triangleright$ $n_Q$ is path node closest to $n_q$
\STATE Initialize path risk $\rho_{\text{path}}$ and distance $d_{\text{path}}$ to 0
\FOR {action $e_{ij}$ in path $a^{-}_{Q:N}$}
\STATE $\rho_{\text{path}}$ += $\rho_{ij} / d_{ij}$; \; $d_{\text{path}}$ += $d_{ij}$
\IF{$\rho_{\text{path}} > \rho_{\text{max}}$ or $d_{\text{path}} > d_{\text{max}}$} 
\STATE Assign root node $n_{\tau} \gets n_i$
\STATE Find root orientation $\mu_{\tau}$ $\triangleright$ if $n_{\tau} = n_Q$, then $\mu_{\tau} \gets \mu$
\RETURN $n_{\tau}$, $\mu_{\tau}$
\ENDIF{}
\ENDFOR{}
\end{algorithmic}


\vspace*{0.1em}


\begin{algorithmic}
\STATE \underbar{\textbf{Function MCTS}}
\STATE \textbf{Input: }state \state \\
\hspace*{2.8em} coverage mask $\{ m_{i} \}$ \\
\vspace*{0.25em}
\STATE Initialize empty lookahead tree $T_r$
\REPEAT
    \item $T_r \gets \textsc{SIMULATE}\big(s; \; \mathcal{G}\big)$
    \item \hspace*{1em} $\triangleright$ estimate generative model $\mathcal{G}$ using efficient
    \item \hspace*{2em} $\text{econGEN}(s, \{ m_i \}, \pi_{rollout})$ in  Alg.~\ref{alg:GenModels}
\UNTIL{timeout}
\RETURN $T_r$
\end{algorithmic}


\end{algorithm}


    
    
    
    




==> fig_probabilistic.tex <==
\begin{figure}[t]
  \centering
  \subfloat[Pessimistic Coverage Model (Deterministic) ]{\label{fig:a}\includegraphics[width=.45\textwidth]{figures/small_fov_combined.png}}
  \; \;
  \subfloat[Optimistic Coverage Model (Deterministic)]{\label{fig:b}\includegraphics[width=.45\textwidth]{figures/big_fov_combined.png}} 
  
  \subfloat[Proposed Probabilistic Coverage Model]{\label{fig:a}\includegraphics[width=.45\textwidth]{figures/prob_fov_combined.png}}

  \caption[The short caption]{\blue{[REMOVE?]} Illustrative example of the effect of different simulated coverage observations on exploration efficiency and completeness: pessimistic observation where the coverage range underestimates true range (a), optimistic observation where the coverage range overestimates true range (b), and our proposed probabilistic observation (c). With the pessimistic model, the robot uncovers the narrow channel after executing an inefficient ping-pong trajectory, which poses undue risk given its occasional proximity to obstacles. Alternatively, the optimistic model leads to an efficient path down the centerline of the cavern, but the robot fails to detect the narrow channel and terminates exploration early. Our proposed probabilistic model combines the benefits of pessimistic and optimistic coverage. The robot travels down the centerline, sparsely covering the main cavern until it encounters the end. At this point, it densely covers the space and exposes the narrow channel.}
  \label{fig:prob_cartoon}
\end{figure}
